Removing supervision in semantic segmentation with local-global matching and area balancing

Removing supervision in semantic segmentation is still tricky. Current approaches can deal with common categorical patterns yet resort to multi-stage architectures. We design a novel end-to-end model leveraging local-global patch matching to predict categories, good localization, area and shape of objects for semantic segmentation. The local-global matching is, in turn, compelled by optimal transport plans fulfilling area constraints nearing a solution for exact shape prediction. Our model attains state-of-the-art in Weakly Supervised Semantic Segmentation, only image-level labels, with 75% mIoU on PascalVOC2012 val set and 46% on MS-COCO2014 val set. Dropping the image-level labels and clustering self-supervised learned features to yield pseudo-multi-level labels, we obtain an unsupervised model for semantic segmentation. We also attain state-of-the-art on Unsupervised Semantic Segmentation with 43.6% mIoU on PascalVOC2012 val set and 19.4% on MS-COCO2014 val set. The code is available at https://github.com/deepplants/PC2M.

==> Images/figure.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> Tables_and_Graphs/old_stuff.tex <==
\begin{table}[h]
  \scriptsize
     \centering
       \resizebox{0.7\columnwidth}{!}
     {%
       \begin{tabular}{|c | c | c | }
         \multicolumn{4}{c}{}\\
         \hline 
         \rowcolor[gray]{.85}
         Method &  PascalVOC2012 &  COCO2014    \\ %[0.5ex]
         \hline
         \hline
         ViT-S/16 & $\times$ & \checkmark  & 35.12 \\
         & \checkmark &  $\times$ & 61.42 \\%\cline{2-4}
         & \checkmark & \checkmark & 69.05 \\
         %\hline
         ViT-B/8 & \checkmark &  \checkmark & 73.12 \\
         ViT-B/16 & \checkmark &  \checkmark & \textbf{75.56} \\
         ViT-L/16 & \checkmark &  \checkmark & 75.24 \\
         %\hline
         \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \end{tabular}}
     \caption{mIoU(\%) score with different configurations on PascalVOC2012 \textit{val} set without CRF.}
     \label{tab:abl}
\end{table}




          ViT-S/16 & \checkmark & 69.05 \\
         %\hline
         ViT-B/8  &  \checkmark & 73.12 \\
         ViT-B/16 &  \checkmark & \textbf{75.56} \\
         ViT-L/16 &  \checkmark & 75.24 \\
         %\hline

==> Tables_and_Graphs/prova.tex <==
\begin{table}[h]
\resizebox{0.7\columnwidth}{!}
    \begin{subtable}[h]{0.12\textwidth}
        \centering
        \begin{tabular}{l | l | l}
        Day & Max Temp & Min Temp \\
        \hline \hline
        Mon & 20 & 13\\
        Tue & 22 & 14\\
        Wed & 23 & 12\\
        Thurs & 25 & 13\\
        Fri & 18 & 7\\
        Sat & 15 & 13\\
        Sun & 20 & 13
       \end{tabular}
       \caption{First Week}
       \label{tab:week1}
    \end{subtable}
    \hfill
    \resizebox{0.7\columnwidth}{!}
    \begin{subtable}[h]{0.12\textwidth}
        \centering
        \begin{tabular}{l | l | l}
        Day & Max Temp & Min Temp \\
        \hline \hline
        Mon & 17 & 11\\
        Tue & 16 & 10\\
        Wed & 14 & 8\\
        Thurs & 12 & 5\\
        Fri & 15 & 7\\
        Sat & 16 & 12\\
        Sun & 15 & 9
        \end{tabular}
        \caption{Second Week}
        \label{tab:week2}
     \end{subtable}
     \caption{Max and min temps recorded in the first two weeks of July}
     \label{tab:temps}
\end{table}

==> Tables_and_Graphs/table_ablations.tex <==
\begin{table}[h]
  \scriptsize
     \centering
       \resizebox{0.7\columnwidth}{!}
     {%
       \begin{tabular}{|c | c | c | c | }
         \multicolumn{4}{c}{}\\
         \hline 
         \rowcolor[gray]{.85}
         Backbone &  OT & Trade &  Results    \\ %[0.5ex]
         \hline
         \hline
         ViT-S/16 & $\times$ & \checkmark  & 35.12 \\
         & \checkmark &  $\times$ & 61.42 \\%\cline{2-4}
         & \checkmark & \checkmark & 69.05 \\
         %\hline
         ViT-B/8 & \checkmark &  \checkmark & 73.12 \\
         ViT-B/16 & \checkmark &  \checkmark & \textbf{75.56} \\
         ViT-L/16 & \checkmark &  \checkmark & 75.24 \\
         %\hline
         \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \end{tabular}}
     \caption{mIoU(\%) score with different configurations on PascalVOC2012 \textit{val} set without CRF.}
     \label{tab:abl}
\end{table}
 
 

==> convergence.tex <==
\noindent
In the main paper, we considered the optimal transport problem with entropic regularization \cite{peyre2019computational}:
\begin{equation}\label{eq:OT}
\displaystyle{
L^{\epsilon}_S({\boldsymbol \delta}, {\boldsymbol \alpha}) = \min_{Q\in U({\boldsymbol \delta}, {\boldsymbol \alpha})} tr(Q^{\top}S) -\epsilon H(Q) }
\end{equation}
\noindent
for both the branches of the network, with costs  $S^{\ell}$ and $S^g$. 
Note that the costs $S^{\ell} {=}{-}\log(P^{\ell})$ and $S^{g} {=}{-}\log(P^{g})$ are both convex and bound. In fact $0{<} P^{\ell},P^{g}{<} 1$.

\noindent 
Nevertheless, the proposed costs are not metrics, which means that, in our case, we cannot consider OT a metric. Our objective  is specifically on the transportation plans $Q^{\ell}$ and $Q^{g}$, which we treat as pseudo-labels in the loss ${\mathcal L}_{trade}$  to constrain the  network predictions.

\noindent
We have specified the average area distribution $\tilde{\alpha}$ as :
\begin{equation}\label{eq:alpha}
\tilde{\alpha_0}^{\ell} {=}\tilde{\alpha_0}^{g} {=}\frac{1}{|C|} \mathds{1}_{|C|}
\mbox{ and }
\Tilde{\alpha}_m^c {=}  (1{-}\gamma) \Tilde{\alpha}_{m{-}1}^c  {+} \gamma \frac{1}{T}\sum_{X{\in}D} q_{m-1}^c(X)
\end{equation}
with $q_m^c(X){=}\displaystyle{\frac{1}{K}\sum_{k=1}^{K} p(y_k{=}c| u_k,F,W^c)}$
 
\noindent
Thus we have two optimal transport problems:
\begin{equation}\label{eq:OT2}
\displaystyle{
L^{\epsilon}_{S^{\ell}}({\boldsymbol \delta}, {\boldsymbol \alpha}^{\ell}) \mbox{ and }
L^{\epsilon}_{S^{g}}({\boldsymbol \delta}, {\boldsymbol \alpha}^{g})}  
\end{equation}
\noindent
We show that:\\
1) $\tilde{\alpha}^{\ell} = \tilde{\alpha}^g$.  

\noindent
2) $Q^{\ell} \neq Q^g$.

\noindent
3) If $\tilde{\alpha}^c_m = \tilde{\alpha}^c_{m-1}$ then
 \begin{equation}\label{eq:converg2}
\Tilde{\alpha}_m^c = \Tilde{\alpha}_{m{-}1}^c = \frac{1}{T}\sum_{X{\in}D} q_{m-1}^c(X) = \frac{1}{T{\cdot} K}\sum_{j\in T\cdot K} P_j^c.
\end{equation}   
 

\noindent
We first prove 1). 
\begin{proof}
We recall $\tilde{\alpha}$ is computed off-line at each epoch on the dataset current predictions.
With a straightforward induction, since $\tilde{\alpha}_0^{\ell} {=} \tilde{\alpha}_0^g {=}\frac{1}{|C|} \mathds{1}_{|C|}$, and since $\gamma$ is fixed, we have that $\tilde{\alpha}^{\ell}_{m{-}1} {=}\tilde{\alpha}_{m{-}1}^g$.  
\noindent
By  definition,  $q_{m}^c(X)$  is the prediction map for $X$, namely, the probability for any patch of the input image $X$ to belong to class $c$, $c{\in} C$, obtained as  the output prediction of the network, via ${\mathcal L}_{PC2M}$, at the current epoch $m$. And here, we are considering all images in the dataset $D$. It follows that $q_{m}^c(X)$ is equal for both  branches, for all $c\in C$. Therefore $\tilde{\alpha}_{m}^{\ell} {=} \tilde{\alpha}_{m}^g$ for all $m$. 
\end{proof}

\noindent
Next, we prove 2). 
\begin{proof}
Suppose $Q^{\ell} = Q^{g}$ and they both are transport plans satisfying eq.~\ref{eq:OT}. Then, according to eq.~\ref{eq:OT}, it must be that 
$(Q^{\ell})^{\top}S^{\ell} {=} (Q^g)^{\top}S^g$, and therefore that $S^{\ell} {=} S^g$.
Since  $S^{\ell} {=} {-}\log(P^{\ell})$ and $S^{g} {=} {-}\log (P^{g})$, and $P^{\ell}$ and $P^g$ are the predictions from the two branches of the network, under the hypothesis that $P^{\ell}$ and $P^g$ are different, due to different augmentations in the two branches, it follows that $S^{\ell} {\neq} S^g$, hence the $Q^{\ell}$ and $Q^g$ minimizing eq. \ref{eq:OT} must be such that $Q^{\ell} {\neq} Q^{g}$.
\end{proof}

\noindent
Here we prove 3). 
\begin{proof}
Suppose $\tilde{\alpha}^c_m {=}\tilde{\alpha}^c_{m-1}$,  by simple manipulations of eq. \ref{eq:alpha}, it follows that $\tilde{\alpha}^c_m {=} \frac{1}{T}\sum_{X{\in}D} q_{m-1}^c(X)$. Here $c$ is any $c{\in} C$.

\noindent
By definition of optimal transport and by 1) above, this implies that $\tilde{\alpha}_m$ is the marginal of $Q^{\ell}$ and also the marginal of $Q^{g}$. 
On the other hand,  $P_j^c$ is the estimated probability of the patches at the network output via ${\mathcal L}_{PC2M}$, therefore
$\Tilde{\alpha}_{m}^c {=} \frac{1}{T}\sum_{X{\in}D}q_{m-1}^c(X) {=} \frac{1}{T{\cdot} K}\sum_{j{\in} T{\cdot} K} P_j^{c}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Figure EMA evolution
\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
    title style={},
    xlabel={epochs},
    ylabel={distance ({\tiny${\times}10^{{-}1}$})},
    xmin=-2, xmax=52,
    ymin=-0.01, ymax=0.31,
    tick align=outside,
    xtick={0, 10, 20, 30, 40, 50},
    ytick={0, 0.1, 0.2, 0.3},
    legend pos=north east,
    ymajorgrids=true,
    xmajorgrids=true,
    grid style=dotted,
    width=5.5cm,
    height=4.5cm,
    label style = {font=\scriptsize},
    %tick style = {font=\scriptsize},
    legend style={nodes={scale=0.4, transform shape}},
    tick label style = {font=\tiny},
    ylabel style={yshift=-0.5cm},
    xlabel style={yshift=0.2cm},
    every major tick/.append style={thick, major tick length=2pt, black},
    xtick pos=left,
    ytick pos=left,
    legend image post style={scale=0.5},
]
\addplot[
    color=blue,
    mark=*,
    mark options={solid},
    mark size=1pt
    ]
    coordinates {
    (0,0.127) (10,0.06) (20, 0.041) (30, 0.03) (40, 0.025) (50, 0.023)
    };
    \addlegendentry{$D_{JS}(\Tilde{\alpha}_{m}{\parallel} \Tilde{\alpha}_{m-1})$}
\addplot[
    color=red,
    mark=*,
    mark options={solid},
    mark size=1pt
    ]
    coordinates {
    (0,0.29) (10, 0.13) (20, 0.083) (30, 0.067) (40, 0.060) (50, 0.057)
    };
    \addlegendentry{$D_{JS}(\alpha^*{\parallel} \Tilde{\alpha}_m)$}
\end{axis}
\end{tikzpicture}
\caption{\scriptsize Evolution of the EMA update for $\gamma{=}0.02$. The blue line shows the distance of $\Tilde{\alpha}_{m}$  to $\Tilde{\alpha}_{m{-}1}$ at epoch $m$, with $\Tilde{\alpha}_{0}$ uniform. The red line shows $\Tilde{\alpha}_{m}$ convergence to ground-truth normalized area distribution of categories $\alpha^*$.  }
\label{fig:alpha_plot}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
Since $\frac{1}{T{\cdot} K}\sum_{j\in T\cdot K} P_j^{c}$ is the network output, by the fact that the marginal of $P$ is equal to the  marginal of both $Q^{\ell}$ and $Q^g$ it follows that at the minimum of the relative entropy\footnote{Here we used the definition as given in \cite{Cover2006}.},  also the marginals of $P^{\ell}$ and $P^{g}$ are both $\tilde{\alpha}_m$.  
As shown in the main paper, since the cost $S^{\ell}{=} {-}\log\left(P^{\ell}\right)^{1/\epsilon} $ and the cost $S^{g}{=} {-}\log\left(P^{g}\right)^{1/\epsilon}$, the Sinkhorn algorithm stops updating. In fact,  the 
update, for $t{\in}\{g,l\}$, is $\mbox{diag}({\bf u}) (P^{t})^{1/\epsilon}\mbox{diag}({\bf v}) ({\mathds 1}_{|C|}){=} {\boldsymbol \delta}$ and $\mbox{diag}({\bf v})[(P^{t})^{1/\epsilon}]^{\top}\mbox{diag}({\bf u})({\mathds 1}_{TK}) {=} {\boldsymbol \tilde{\alpha}_m}$ which is already satisfied  for the unknown variables $({\bf u}, {\bf v}){=} ({\mathds 1}_{TK},{\mathds 1}_{|C|})$, and  the hypothesis that $\epsilon {\approx}1$ towards the end of training. \end{proof}

\subsection{Empirical convergence of {\larger $\alpha$} to ground truth average areas}\label{sub-sec:empirical}
Given the above statements, it is natural to ask whether the average area $\tilde{\alpha}$ converges to the ground truth average area
 $\alpha^{*} {=} (\frac{1}{T} \sum_{j\in T} A_j^{c},\ldots,\frac{1}{T} \sum_{j\in T} A_j^{|C|})^{\top}$, we 
 show experimentally that $\|\tilde{\alpha}{-}\alpha^{*}\|{<}\lambda$.

\noindent
Figure \ref{fig:alpha_plot} shows the evolution during training of the estimated average area distribution of categories for the PascalVOC2012\cite{everingham2010pascal} \textit{trainaug} dataset \cite{hariharan2011semantic}, using $\gamma=0.02$ for EMA update (see eq.~{\color{red} 7}  in the main paper). Namely, we use Jensen–Shannon divergence ($D_{JS}$) to assess the similarity between distributions. The red line in Figure \ref{fig:alpha_plot} shows the divergence at epoch $m$ between $\tilde{\alpha}_{m}$ and the ground truth area distribution of categories $\alpha^*$. 
This show, experimentally, that $\|\tilde{\alpha} {-}\alpha^{*}\|{<}\lambda$, for $\lambda {<}0.05$. The blue line in Figure \ref{fig:alpha_plot} shows the convergence of the slow-moving distribution $\Tilde{\alpha}$ to a fixed target, that is, we compute the divergence at epoch $m$ between $\Tilde{\alpha}_m$ and $\Tilde{\alpha}_{m-1}$ to assess the magnitude of change of the distribution during the epochs. A similar graph can be shown between $\Tilde{\alpha}_m$ and  $\frac{1}{T}\sum_{X{\in}D} q_{m-1}^c(X)$. 

\noindent
In particular, as stated in eq.~{\color{red} 5} in the main paper $\alpha$, which is used in Algorithm \ref{problem:algo}, is defined to be $\frac{\nu_B}{Z\nu_D}\tilde{\alpha}$, with  $\nu_B$ the frequency of categories in the batch, here equal to 1 to obtain the unitary average area. Noticing that $\nu_D$ is a constant, it follows that the above results also holds for $Z\alpha$.
Therefore, in \Cref{fig:alpha_dist} we show that the above-assessed similarity is consistently extended to $\|\alpha^c{-}\alpha^{c,*}\|{<}\lambda$ up to a multiplicative factor proportional to  $Z$, for all $c\in C$.


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{Images/alpha.png}
    \caption{Temporal evolution of estimated unitary area distribution $\Tilde{\boldsymbol\alpha}_m/{\boldsymbol\nu_D}$ at epochs $m=\{0,20,50\}$ on PascalVOC2012 \textit{trainaug} set. $\Tilde{\boldsymbol\alpha}$ is the categories' area distribution, $\boldsymbol\nu_D$ is the relative class frequency, and $\boldsymbol\alpha^\star$ is the ground truth categories' area distribution in the dataset.}
    \label{fig:alpha_dist}
\end{figure*}


